Major Substructure in the M31 Outer Halo: the East Cloud

We present the first detailed analysis of the East Cloud, a highly disrupted diffuse stellar substructure in the outer halo of M31. The core of the substructure lies at a projected distance of $\sim100$ kpc from the centre of M31 in the outer halo, with possible extensions reaching right into the inner halo. Using Pan-Andromeda Archaeological Survey photometry of red giant branch stars, we measure the distance, metallicity and brightness of the cloud. Using Hubble Space Telescope data, we independently measure the distance and metallicity to the two globular clusters coincident with the East Cloud core, PA-57 and PA-58, and find their distances to be consistent with the cloud. Four further globular clusters coincident with the substructure extensions are identified as potentially associated. Combining the analyses, we determine a distance to the cloud of $814^{+20}_{-9}$ kpc, a metallicity of $[Fe/H] = -1.2\pm0.1$, and a brightness of $M_V = -10.7\pm0.4$ mag. Even allowing for the inclusion of the potential extensions, this accounts for less than $20$ per cent of the progenitor luminosity implied by the luminosity-metallicity relation. Using the updated techniques developed for this analysis, we also refine our estimates of the distance and brightness of the South-West Cloud, a separate substructure analyzed in the previous work in this series.

==> Makefile <==
filename=ecloud_revised

pdf:
	pdflatex --shell-escape --enable-write18 ${filename}
	bibtex ${filename}||true
	pdflatex --shell-escape --enable-write18 ${filename}
	pdflatex --shell-escape --enable-write18 ${filename}
#shell escape is for epstopdf to work (also make sure graphics is does not have any options specified (which may conflict with epstopdf options), by putting graphics in as a \usepackage{} command)
#For large images: save as png, convert to pdf (convert file.png file.pdf)
#If necessary, convert to eps using "pdftops -eps file.pdf" (better compression than convert)


read:
	evince ${filename}.pdf &

aread:
	acroread ${filename}.pdf &

clean:
	rm -f ${filename}.ps ${filename}.pdf ${filename}.log ${filename}.aux ${filename}.out ${filename}.dvi ${filename}.bbl ${filename}.blg

retarget: 
	sed 's/^filename=.*/filename=${TARGET}/g' -i ./Makefile
#overwrites lines starting with filename= with filename=${TARGET}
#usage: make TARGET=<new filename> retarget


